Non-Uniform Cellular Automata: classes, dynamics, and decidability

The dynamical behavior of non-uniform cellular automata is compared with the one of classical cellular automata. Several differences and similarities are pointed out by a series of examples. Decidability of basic properties like surjectivity and injectivity is also established. The final part studies a strong form of equicontinuity property specially suited for non-uniform cellular automata.

==> DeBruijn2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Jun 18 15:27:15 CEST 2009
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-12.5" x-max="142.5" y-min="0" y-max="135" auto-bounding="true">
%<g>
%<ellipse fill-style= "none"
%	 p3= "(30,50)"
%	 p2= "(30,60)"
%	 p1= "(20,60)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(25,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$00,0$
%</text>
%<ellipse fill-style= "none"
%	 p3= "(50,30)"
%	 p2= "(50,40)"
%	 p1= "(40,40)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "none"
%	 p3= "(10,30)"
%	 p2= "(10,40)"
%	 p1= "(0,40)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "none"
%	 p3= "(30,10)"
%	 p2= "(30,20)"
%	 p1= "(20,20)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(5,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$10,0$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(25,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$11,0$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(45,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$01,0$
%</text>
%<smoothpolygon fill-style= "none"
%	 closed= "false"
%	 points= "(5,40);(7.5,52.5);(20,55)"
%	 right-arrow= "head"
%	 smoothness= "0.7;0.7;0.7"
%	 />
%<smoothpolygon fill-style= "none"
%	 closed= "false"
%	 points= "(30,55);(42.5,52.5);(45,40)"
%	 right-arrow= "head"
%	 smoothness= "0.7;0.7;0.7"
%	 />
%<smoothpolygon fill-style= "none"
%	 closed= "false"
%	 points= "(45,30);(42.5,17.5);(30,15)"
%	 right-arrow= "head"
%	 smoothness= "0.7;0.7;0.7"
%	 />
%<smoothpolygon fill-style= "none"
%	 closed= "false"
%	 points= "(20,15);(7.5,17.5);(5,30)"
%	 right-arrow= "head"
%	 smoothness= "0.7;0.7;0.7"
%	 />
%<smoothpolygon fill-style= "none"
%	 closed= "false"
%	 points= "(22.5,60);(18.75,63.75);(25,68.75);(31.25,63.75);(27.5,60)"
%	 right-arrow= "head"
%	 smoothness= "0.7;0.7;0.7;0.7;0.7"
%	 />
%<smoothpolygon fill-style= "none"
%	 closed= "false"
%	 points= "(27.5,10);(31.25,6.25);(25,1.25);(18.75,6.25);(22.5,10)"
%	 right-arrow= "head"
%	 smoothness= "0.7;0.7;0.7;0.7;0.7"
%	 />
%<smoothpolygon fill-style= "none"
%	 closed= "false"
%	 points= "(10,37.5);(25,45);(40,37.5)"
%	 right-arrow= "head"
%	 smoothness= "0.7;0.7;0.7"
%	 />
%<smoothpolygon fill-style= "none"
%	 closed= "false"
%	 points= "(40,32.5);(25,25);(10,32.5)"
%	 right-arrow= "head"
%	 smoothness= "0.7;0.7;0.7"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(6.25,52.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$(1,0)$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(25,43.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$(1,0)$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(6.25,17.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$(1,0)$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(25,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$(1,0)$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(25,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$(0,0)$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(43.75,52.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$(0,0)$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(43.75,17.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$(0,0)$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(25,26.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$(0,0)$
%</text>
%</g>
%<g>
%<ellipse fill-style= "none"
%	 p3= "(110,50)"
%	 p2= "(110,60)"
%	 p1= "(100,60)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(105,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$00,1$
%</text>
%<ellipse fill-style= "none"
%	 p3= "(130,30)"
%	 p2= "(130,40)"
%	 p1= "(120,40)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "none"
%	 p3= "(90,30)"
%	 p2= "(90,40)"
%	 p1= "(80,40)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "none"
%	 p3= "(110,10)"
%	 p2= "(110,20)"
%	 p1= "(100,20)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(85,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$10,1$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(105,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$11,1$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(125,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$01,1$
%</text>
%<smoothpolygon fill-style= "none"
%	 closed= "false"
%	 points= "(85,40);(87.5,52.5);(100,55)"
%	 right-arrow= "head"
%	 smoothness= "0.7;0.7;0.7"
%	 />
%<smoothpolygon fill-style= "none"
%	 closed= "false"
%	 points= "(110,55);(122.5,52.5);(125,40)"
%	 right-arrow= "head"
%	 smoothness= "0.7;0.7;0.7"
%	 />
%<smoothpolygon fill-style= "none"
%	 closed= "false"
%	 points= "(125,30);(123.75,18.75);(110,15)"
%	 right-arrow= "head"
%	 smoothness= "0.7;0.7;0.7"
%	 />
%<smoothpolygon fill-style= "none"
%	 closed= "false"
%	 points= "(100,15);(87.5,17.5);(85,30)"
%	 right-arrow= "head"
%	 smoothness= "0.7;0.7;0.7"
%	 />
%<smoothpolygon fill-style= "none"
%	 closed= "false"
%	 points= "(102.5,60);(98.75,63.75);(105,68.75);(111.25,63.75);(107.5,60)"
%	 right-arrow= "head"
%	 smoothness= "0.7;0.7;0.7;0.7;0.7"
%	 />
%<smoothpolygon fill-style= "none"
%	 closed= "false"
%	 points= "(107.5,10);(111.25,6.25);(105,1.25);(98.75,6.25);(102.5,10)"
%	 right-arrow= "head"
%	 smoothness= "0.7;0.7;0.7;0.7;0.7"
%	 />
%<smoothpolygon fill-style= "none"
%	 closed= "false"
%	 points= "(90,37.5);(105,45);(120,37.5)"
%	 right-arrow= "head"
%	 smoothness= "0.7;0.7;0.7"
%	 />
%<smoothpolygon fill-style= "none"
%	 closed= "false"
%	 points= "(120,32.5);(105,25);(90,32.5)"
%	 right-arrow= "head"
%	 smoothness= "0.7;0.7;0.7"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(86.25,52.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$(0,1)$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(105,43.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$(1,1)$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(86.25,17.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$(0,1)$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(105,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$(1,1)$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(105,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$(0,1)$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(123.75,52.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$(1,1)$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(123.75,17.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$(1,1)$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(105,26.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$(0,1)$
%</text>
%</g>
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(50,35);(50,35);(80,35);(80,35)"
%	 right-arrow= "head"
%	 />
%<smoothpolygon fill-style= "none"
%	 stroke-color= "#ff0000"
%	 closed= "false"
%	 points= "(48.75,31.25);(70,10);(100,12.5)"
%	 right-arrow= "head"
%	 smoothness= "0.7;0.7;0.7"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(65,37.5)"
%	 stroke-color= "#ff0000"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\textcolor{red}{(1,0)}$
%</text>
%<smoothpolygon fill-style= "none"
%	 stroke-color= "#ff0000"
%	 closed= "false"
%	 points= "(30,12.5);(65,5);(100,11.25)"
%	 right-arrow= "head"
%	 smoothness= "0.7;0.7;0.7"
%	 />
%<smoothpolygon fill-style= "none"
%	 stroke-color= "#ff0000"
%	 closed= "false"
%	 points= "(30,13.75);(70,13.75);(81.25,31.25)"
%	 right-arrow= "head"
%	 smoothness= "0.7;0.7;0.7"
%	 />
%<smoothpolygon fill-style= "none"
%	 stroke-color= "#ff0000"
%	 closed= "false"
%	 points= "(8.75,38.75);(43.75,60);(72.5,65);(100,57.5)"
%	 right-arrow= "head"
%	 smoothness= "0.7;0.7;0.7;0.7"
%	 />
%<smoothpolygon fill-style= "none"
%	 stroke-color= "#ff0000"
%	 closed= "false"
%	 points= "(30,57.5);(73.75,80);(101.25,58.75)"
%	 right-arrow= "head"
%	 smoothness= "0.7;0.7;0.7"
%	 />
%<smoothpolygon fill-style= "none"
%	 stroke-color= "#ff0000"
%	 closed= "false"
%	 points= "(28.75,58.75);(47.5,77.5);(86.25,81.25);(118.75,76.25);(137.5,56.25);(128.75,38.75)"
%	 right-arrow= "head"
%	 smoothness= "0.7;0.7;0.7;0.7;0.7;0.7"
%	 />
%<smoothpolygon fill-style= "none"
%	 stroke-color= "#ff0000"
%	 closed= "false"
%	 points= "(2.5,40);(0,62.5);(17.5,81.25);(42.5,88.75);(75,91.25);(113.75,86.25);
%	(133.75,76.25);(142.5,61.25);(138.75,43.75);(130,36.25)"
%	 right-arrow= "head"
%	 smoothness= "0.7;0.7;0.7;0.7;0.7;0.7;0.7;0.7;0.7;0.7"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(77.5,92.5)"
%	 stroke-color= "#ff0000"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\textcolor{red}{(0,0)}$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(85,82.5)"
%	 stroke-color= "#ff0000"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\textcolor{red}{(0,0)}$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(52.5,63.75)"
%	 stroke-color= "#ff0000"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\textcolor{red}{(0,0)}$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(70,72.5)"
%	 stroke-color= "#ff0000"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\textcolor{red}{(0,0)}$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(65,11.25)"
%	 stroke-color= "#ff0000"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\textcolor{red}{(1,0)}$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(55,18.75)"
%	 stroke-color= "#ff0000"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\textcolor{red}{(1,0)}$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(77.5,17.5)"
%	 stroke-color= "#ff0000"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\textcolor{red}{(1,0)}$
%</text>
%<g>
%<smoothpolygon fill-style= "none"
%	 closed= "false"
%	 points= "(-5,110);(-10,112.5);(-12.5,120);(-10,127.5);(-5,130)"
%	 right-arrow= "head"
%	 smoothness= "0.7;0.7;0.7;0.7;0.7"
%	 />
%<g>
%<parallelogram fill-style= "none"
%	 p3= "(72.5,135)"
%	 p2= "(72.5,125)"
%	 p1= "(62.5,125)"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(82.5,135)"
%	 p2= "(82.5,125)"
%	 p1= "(72.5,125)"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(92.5,135)"
%	 p2= "(92.5,125)"
%	 p1= "(82.5,125)"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(102.5,135)"
%	 p2= "(102.5,125)"
%	 p1= "(92.5,125)"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(122.5,135)"
%	 p2= "(122.5,125)"
%	 p1= "(112.5,125)"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(112.5,135)"
%	 p2= "(112.5,125)"
%	 p1= "(102.5,125)"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(22.5,135)"
%	 p2= "(22.5,125)"
%	 p1= "(12.5,125)"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(32.5,135)"
%	 p2= "(32.5,125)"
%	 p1= "(22.5,125)"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(42.5,135)"
%	 p2= "(42.5,125)"
%	 p1= "(32.5,125)"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(62.5,135)"
%	 p2= "(62.5,125)"
%	 p1= "(52.5,125)"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(52.5,135)"
%	 p2= "(52.5,125)"
%	 p1= "(42.5,125)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(122.5,135);(122.5,135);(132.5,135);(132.5,135)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(122.5,125);(122.5,125);(132.5,125);(132.5,125)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,135);(2.5,135);(12.5,135);(12.5,135)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,125);(2.5,125);(12.5,125);(12.5,125)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-style= "dashed"
%	 stroke-dasharray= "1;1"
%	 points= "(127.5,130);(127.5,130);(137.5,130);(137.5,130)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-style= "dashed"
%	 stroke-dasharray= "1;1"
%	 points= "(-2.5,130);(-2.5,130);(7.5,130);(7.5,130)"
%	 />
%</g>
%<g>
%<parallelogram fill-style= "none"
%	 p3= "(72.5,115)"
%	 p2= "(72.5,105)"
%	 p1= "(62.5,105)"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(82.5,115)"
%	 p2= "(82.5,105)"
%	 p1= "(72.5,105)"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(92.5,115)"
%	 p2= "(92.5,105)"
%	 p1= "(82.5,105)"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(102.5,115)"
%	 p2= "(102.5,105)"
%	 p1= "(92.5,105)"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(122.5,115)"
%	 p2= "(122.5,105)"
%	 p1= "(112.5,105)"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(112.5,115)"
%	 p2= "(112.5,105)"
%	 p1= "(102.5,105)"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(22.5,115)"
%	 p2= "(22.5,105)"
%	 p1= "(12.5,105)"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(32.5,115)"
%	 p2= "(32.5,105)"
%	 p1= "(22.5,105)"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(42.5,115)"
%	 p2= "(42.5,105)"
%	 p1= "(32.5,105)"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(62.5,115)"
%	 p2= "(62.5,105)"
%	 p1= "(52.5,105)"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(52.5,115)"
%	 p2= "(52.5,105)"
%	 p1= "(42.5,105)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(122.5,115);(122.5,115);(132.5,115);(132.5,115)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(122.5,105);(122.5,105);(132.5,105);(132.5,105)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,115);(2.5,115);(12.5,115);(12.5,115)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,105);(2.5,105);(12.5,105);(12.5,105)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-style= "dashed"
%	 stroke-dasharray= "1;1"
%	 points= "(127.5,110);(127.5,110);(137.5,110);(137.5,110)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-style= "dashed"
%	 stroke-dasharray= "1;1"
%	 points= "(-2.5,110);(-2.5,110);(7.5,110);(7.5,110)"
%	 />
%</g>
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(67.5,115);(67.5,115);(67.5,125);(67.5,125)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(127.5,115);(127.5,115);(117.5,125);(117.5,125)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(117.5,115);(117.5,115);(107.5,125);(107.5,125)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(107.5,115);(107.5,115);(97.5,125);(97.5,125)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(97.5,115);(97.5,115);(87.5,125);(87.5,125)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(87.5,115);(87.5,115);(77.5,125);(77.5,125)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(7.5,115);(7.5,115);(17.5,125);(17.5,125)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(17.5,115);(17.5,115);(27.5,125);(27.5,125)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(27.5,115);(27.5,115);(37.5,125);(37.5,125)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(37.5,115);(37.5,115);(47.5,125);(47.5,125)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(47.5,115);(47.5,115);(57.5,125);(57.5,125)"
%	 right-arrow= "head"
%	 />
%</g>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(142.5,135)
\rput{0}(25,55){\psellipse[](0,0)(5,-5)}
\rput(25,55){$00,0$}
\rput{0}(45,35){\psellipse[](0,0)(5,-5)}
\rput{0}(5,35){\psellipse[](0,0)(5,-5)}
\rput{0}(25,15){\psellipse[](0,0)(5,-5)}
\rput(5,35){$10,0$}
\rput(25,15){$11,0$}
\rput(45,35){$01,0$}
\psbezier{->}(5,40)(6.75,48.75)(11.25,53.25)(20,55)
\psbezier{->}(30,55)(38.75,53.25)(43.25,48.75)(45,40)
\psbezier{->}(45,30)(43.25,21.25)(38.75,16.75)(30,15)
\psbezier{->}(20,15)(11.25,16.75)(6.75,21.25)(5,30)
\pscustom[]{\psbezier{-}(22.5,60)(19.88,62.62)(19.69,64.5)(21.88,66.25)
\psbezier(24.06,68)(25.94,68)(28.12,66.25)
\psbezier{->}(30.31,64.5)(30.12,62.62)(27.5,60)
}
\pscustom[]{\psbezier{-}(27.5,10)(30.12,7.38)(30.31,5.5)(28.12,3.75)
\psbezier(25.94,2)(24.06,2)(21.88,3.75)
\psbezier{->}(19.69,5.5)(19.88,7.38)(22.5,10)
}
\psbezier{->}(10,37.5)(20.5,42.75)(29.5,42.75)(40,37.5)
\psbezier{->}(40,32.5)(29.5,27.25)(20.5,27.25)(10,32.5)
\rput(6.25,52.5){$(1,0)$}
\rput(25,43.75){$(1,0)$}
\rput(6.25,17.5){$(1,0)$}
\rput(25,0){$(1,0)$}
\rput(25,70){$(0,0)$}
\rput(43.75,52.5){$(0,0)$}
\rput(43.75,17.5){$(0,0)$}
\rput(25,26.25){$(0,0)$}
\rput{0}(105,55){\psellipse[](0,0)(5,-5)}
\rput(105,55){$00,1$}
\rput{0}(125,35){\psellipse[](0,0)(5,-5)}
\rput{0}(85,35){\psellipse[](0,0)(5,-5)}
\rput{0}(105,15){\psellipse[](0,0)(5,-5)}
\rput(85,35){$10,1$}
\rput(105,15){$11,1$}
\rput(125,35){$01,1$}
\psbezier{->}(85,40)(86.75,48.75)(91.25,53.25)(100,55)
\psbezier{->}(110,55)(118.75,53.25)(123.25,48.75)(125,40)
\psbezier{->}(125,30)(124.12,22.12)(119.62,17.62)(110,15)
\psbezier{->}(100,15)(91.25,16.75)(86.75,21.25)(85,30)
\pscustom[]{\psbezier{-}(102.5,60)(99.88,62.62)(99.69,64.5)(101.88,66.25)
\psbezier(104.06,68)(105.94,68)(108.12,66.25)
\psbezier{->}(110.31,64.5)(110.12,62.62)(107.5,60)
}
\pscustom[]{\psbezier{-}(107.5,10)(110.12,7.38)(110.31,5.5)(108.12,3.75)
\psbezier(105.94,2)(104.06,2)(101.88,3.75)
\psbezier{->}(99.69,5.5)(99.88,7.38)(102.5,10)
}
\psbezier{->}(90,37.5)(100.5,42.75)(109.5,42.75)(120,37.5)
\psbezier{->}(120,32.5)(109.5,27.25)(100.5,27.25)(90,32.5)
\rput(86.25,52.5){$(0,1)$}
\rput(105,43.75){$(1,1)$}
\rput(86.25,17.5){$(0,1)$}
\rput(105,0){$(1,1)$}
\rput(105,70){$(0,1)$}
\rput(123.75,52.5){$(1,1)$}
\rput(123.75,17.5){$(1,1)$}
\rput(105,26.25){$(0,1)$}
\psline[linecolor=red]{->}(50,35)(80,35)
\psbezier[linecolor=red]{->}(48.75,31.25)(63.62,16.38)(79,10.75)(100,12.5)
\rput(65,37.5){$\textcolor{red}{(1,0)}$}
\psbezier[linecolor=red]{->}(30,12.5)(54.5,7.25)(75.5,6.88)(100,11.25)
\psbezier[linecolor=red]{->}(30,13.75)(58,13.75)(73.38,19)(81.25,31.25)
\pscustom[linecolor=red]{\psbezier{-}(8.75,38.75)(33.25,53.62)(48.06,60.75)(58.12,62.5)
\psbezier{->}(68.19,64.25)(80.75,62.75)(100,57.5)
}
\psbezier[linecolor=red]{->}(30,57.5)(60.62,73.25)(82,73.62)(101.25,58.75)
\pscustom[linecolor=red]{\psbezier{-}(28.75,58.75)(41.88,71.88)(53.31,78.06)(66.88,79.38)
\psbezier(80.44,80.69)(91.12,80.5)(102.5,78.75)
\psbezier(113.88,77)(121.56,73.25)(128.12,66.25)
\psbezier{->}(134.69,59.25)(134.88,51)(128.75,38.75)
}
\pscustom[linecolor=red]{\psbezier{-}(2.5,40)(0.75,55.75)(2.62,65.31)(8.75,71.88)
\psbezier(14.88,78.44)(21.25,82.38)(30,85)
\psbezier(38.75,87.62)(47.38,89.12)(58.75,90)
\psbezier(70.12,90.88)(80.81,90.5)(94.38,88.75)
\psbezier(107.94,87)(116.75,84.75)(123.75,81.25)
\psbezier(130.75,77.75)(135.06,74)(138.12,68.75)
\psbezier(141.19,63.5)(141.94,58.62)(140.62,52.5)
\psbezier{->}(139.31,46.38)(136.12,41.5)(130,36.25)
}
\rput(77.5,92.5){$\textcolor{red}{(0,0)}$}
\rput(85,82.5){$\textcolor{red}{(0,0)}$}
\rput(52.5,63.75){$\textcolor{red}{(0,0)}$}
\rput(70,72.5){$\textcolor{red}{(0,0)}$}
\rput(65,11.25){$\textcolor{red}{(1,0)}$}
\rput(55,18.75){$\textcolor{red}{(1,0)}$}
\rput(77.5,17.5){$\textcolor{red}{(1,0)}$}
\pscustom[]{\psbezier{-}(-5,110)(-8.5,111.75)(-10.38,113.62)(-11.25,116.25)
\psbezier(-12.12,118.88)(-12.12,121.12)(-11.25,123.75)
\psbezier{->}(-10.38,126.38)(-8.5,128.25)(-5,130)
}
\pspolygon[](62.5,125)(72.5,125)(72.5,135)(62.5,135)
\pspolygon[](72.5,125)(82.5,125)(82.5,135)(72.5,135)
\pspolygon[](82.5,125)(92.5,125)(92.5,135)(82.5,135)
\pspolygon[](92.5,125)(102.5,125)(102.5,135)(92.5,135)
\pspolygon[](112.5,125)(122.5,125)(122.5,135)(112.5,135)
\pspolygon[](102.5,125)(112.5,125)(112.5,135)(102.5,135)
\pspolygon[](12.5,125)(22.5,125)(22.5,135)(12.5,135)
\pspolygon[](22.5,125)(32.5,125)(32.5,135)(22.5,135)
\pspolygon[](32.5,125)(42.5,125)(42.5,135)(32.5,135)
\pspolygon[](52.5,125)(62.5,125)(62.5,135)(52.5,135)
\pspolygon[](42.5,125)(52.5,125)(52.5,135)(42.5,135)
\psline(122.5,135)(132.5,135)
\psline(122.5,125)(132.5,125)
\psline(2.5,135)(12.5,135)
\psline(2.5,125)(12.5,125)
\psline[linestyle=dashed,dash=1 1](127.5,130)(137.5,130)
\psline[linestyle=dashed,dash=1 1](-2.5,130)(7.5,130)
\pspolygon[](62.5,105)(72.5,105)(72.5,115)(62.5,115)
\pspolygon[](72.5,105)(82.5,105)(82.5,115)(72.5,115)
\pspolygon[](82.5,105)(92.5,105)(92.5,115)(82.5,115)
\pspolygon[](92.5,105)(102.5,105)(102.5,115)(92.5,115)
\pspolygon[](112.5,105)(122.5,105)(122.5,115)(112.5,115)
\pspolygon[](102.5,105)(112.5,105)(112.5,115)(102.5,115)
\pspolygon[](12.5,105)(22.5,105)(22.5,115)(12.5,115)
\pspolygon[](22.5,105)(32.5,105)(32.5,115)(22.5,115)
\pspolygon[](32.5,105)(42.5,105)(42.5,115)(32.5,115)
\pspolygon[](52.5,105)(62.5,105)(62.5,115)(52.5,115)
\pspolygon[](42.5,105)(52.5,105)(52.5,115)(42.5,115)
\psline(122.5,115)(132.5,115)
\psline(122.5,105)(132.5,105)
\psline(2.5,115)(12.5,115)
\psline(2.5,105)(12.5,105)
\psline[linestyle=dashed,dash=1 1](127.5,110)(137.5,110)
\psline[linestyle=dashed,dash=1 1](-2.5,110)(7.5,110)
\psline[linecolor=red]{->}(67.5,115)(67.5,125)
\psline{->}(127.5,115)(117.5,125)
\psline{->}(117.5,115)(107.5,125)
\psline{->}(107.5,115)(97.5,125)
\psline{->}(97.5,115)(87.5,125)
\psline{->}(87.5,115)(77.5,125)
\psline{->}(7.5,115)(17.5,125)
\psline{->}(17.5,115)(27.5,125)
\psline{->}(27.5,115)(37.5,125)
\psline{->}(37.5,115)(47.5,125)
\psline{->}(47.5,115)(57.5,125)
\end{pspicture}

